Exploring Prompt Patterns in AI-Assisted Code Generation: Towards Faster and More Effective Developer-AI Collaboration

The growing integration of AI tools in software development, particularly Large Language Models (LLMs) such as ChatGPT, has revolutionized how developers approach coding tasks. However, achieving high-quality code often requires iterative interactions, which can be time-consuming and inefficient. This paper explores the application of structured prompt patterns to minimize the number of interactions required for satisfactory AI-assisted code generation. Using the DevGPT dataset, we analyzed seven distinct prompt patterns to evaluate their effectiveness in reducing back-and-forth communication between developers and AI. Our findings highlight patterns such as ''Context and Instruction'' and ''Recipe'' as particularly effective in achieving high-quality outputs with minimal iterations. The study emphasizes the potential for prompt engineering to streamline developer-AI collaboration, providing practical insights into crafting prompts that balance precision, efficiency, and clarity.

==> Tables/Project_Overview.tex <==
\begin{table}[h!]
\begin{center}
\caption{Dataset overview of refactoring-related issues.}

%\anthony{are these all refactoring issues or issues with refactoings in the title? \eman{issues with refactorings in the title}}
\label{Table:DATA_Overview}
\begin{adjustbox}{width=0.35\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lllll}\hline
\toprule
\bfseries Item & \bfseries Count \\
\midrule
Refactoring commits with issues & 45,477 \\
Refactoring commits with issues having keyword `\textit{refactor*}' in title & 835 \\
Refactoring operations associated with issues &  15,833 \\
\midrule
\multicolumn{2}{c}{\textbf{\textit{Issue Status}}}\\
\bfseries Item & \bfseries Count  \\
\midrule
Closed & 603 \\
In progress & 8 \\
Open & 28 \\
Resolved & 196 \\
\midrule
\multicolumn{2}{c}{\textbf{\textit{Issue Resolution}}}\\
\bfseries Item & \bfseries Count  \\
\midrule
Done & 4 \\
Fixed & 780 \\
Implemented & 8 \\
Resolved & 4 \\
Won't fix & 3 \\
\midrule
\multicolumn{2}{c}{\textbf{\textit{Issue Types}}}\\
\bfseries Item & \bfseries Count  \\
\midrule
Bug & 95 \\
Improvement & 390 \\
New Feature & 2\\
Story & 1\\
Sub-task & 71 \\
Task & 274 \\
Test & 2 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}
